Graph Belief Propagation Networks

With the wide-spread availability of complex relational data, semi-supervised node classification in graphs has become a central machine learning problem. Graph neural networks are a recent class of easy-to-train and accurate methods for this problem that map the features in the neighborhood of a node to its label, but they ignore label correlation during inference and their predictions are difficult to interpret. On the other hand, collective classification is a traditional approach based on interpretable graphical models that explicitly model label correlations. Here, we introduce a model that combines the advantages of these two approaches, where we compute the marginal probabilities in a conditional random field, similar to collective classification, and the potentials in the random field are learned through end-to-end training, akin to graph neural networks. In our model, potentials on each node only depend on that node's features, and edge potentials are learned via a coupling matrix. This structure enables simple training with interpretable parameters, scales to large networks, naturally incorporates training labels at inference, and is often more accurate than related approaches. Our approach can be viewed as either an interpretable message-passing graph neural network or a collective classification method with higher capacity and modernized training.

==> paper/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
      \answerYes{See \cref{subsec:practical_considerations}.}
  \item Did you discuss any potential negative societal impacts of your work?
      \answerYes{See \cref{sec:conclusions}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
      \answerYes{See \cref{subsec:additional_implementation,subsec:additional_setup,subsec:additional_datasets}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
      \answerYes{See \cref{subsec:results_full_batch,subsec:subsampling}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerYes{See \cref{tab:results_synthetic_full_batch,tab:results_empirical_full_batch,tab:results_empirical_mini_batch}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \cref{subsec:results_full_batch,subsec:subsampling}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
      \answerYes{In the beginning of \cref{sec:experiments}, we cited the creators of the public datasets and one proprietary dataset. When comparing against the GMNN, DeeperGNN baselines, we cited the original paper.}
  \item Did you mention the license of the assets?
    \answerYes{See page 6 footnote.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See \cref{subsec:additional_implementation,subsec:additional_setup,subsec:additional_datasets}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See \cref{subsec:results_full_batch}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> paper/related_work.tex <==
\section{Additional Related Works}
%
Collective classification or collective inference refers to a set of machine learning algorithms for relational data, that take advantage of the correlation between the features and the labels, as well as labels on the neighboring vertices~\cite{jensen2004collective,sen2008collective,london2014collective}.
%
One class of methods use local conditional classifiers, either iteratively alternates between predicting outcomes for each node and updating the features of each node with predicted outcome on neighboring nodes~\cite{neville2000iterative,lu2003link}, or repeatedly sample the label on each individual node one-by-one, until some equilibrium is reached~\cite{macskassy2007classification,mcdowell2007cautious}.
%
Another class of methods is directly related to our work, where they also use a pairwise MRF as the data model, and the inference algorithm uses belief propagation to compute consensus~\cite{taskar2002discriminative}.
%
The major difference is that they estimate the MRF coupling-potentials by maximizing the joint likelihood of all the nodes, and therefore require a fully labeled graph for training.
%
In contrast, our model is learned discriminatively end-to-end on the training nodes by back-propagating the gradients through belief propagation steps.

Several works have proposed to combine Markov random field and graph neural networks~\cite{qu2019gmnn,ma2019cgnf}.
%
They add a conditional random field layer to model the joint distribution of the node labels, and they maximize the joint probability of the observed labels during training, and require using variational methods or pseudolikelihood to approximate the partition function.
%
In contrast, GBPN avoid those difficulties by optimizing for the marginal likelihood.

Recently, several heuristics have been proposed to directly leverage training labels for inference: 
\circled{1} diffusing training labels along graph topology as additional features~\cite{shi2020masked};
\circled{2} add a random field ``layer'' on top of the GNN model to learn correlated structure in the labels~\cite{gao2019conditional,qu2019gmnn};
\circled{3} post-processing predicted probabilities with training residuals~\cite{jia2020residual,huang2020combining}.
%
These approaches are unsatisfying because they are largely ad hoc, and there is little understanding of why or when one particular approach should work.
%
In comparison, incorporating training labels during inference in GBPN naturally corresponds to conditioning on all available information (both features and training labels) for prediction.

Some recent works consider learning a belief-propagation algorithm to estimate the partition function in a graphical model~\cite{yoon2018inference,kuck2020belief}. In comparison, our work focuses on the node classification problem.

